CTseg: A Tool for Brain CT Segmentation, Spatial Normalisation, and Volumetrics

This paper presents and validates CTseg, a freely available software for brain CT segmentation, spatial normalisation, and volumetrics. CTseg builds on the Multi-Brain generative modelling framework, providing a CT-specific pipeline that produces tissue maps, deformation fields, and brain volume estimates in the same format as SPM's unified segmentation, thereby extending SPM's established analysis chain from MRI to CT. CTseg is designed for routine hospital CT scans without requiring preprocessing or resampling in deployment. Although CTseg has been adopted in clinical research spanning, among other things, stroke, dementia, and brain morphometry, a systematic validation against an independent reference standard has been lacking. Using paired MR/CT head scans, we evaluate CTseg across four dimensions: segmentation accuracy against an MRI-derived silver standard; spatial normalisation consistency through group-average sharpness and voxelwise coefficient of variation; brain volume agreement via intraclass correlation and Bland-Altman analysis; and downstream sex classification performance from normalised tissue maps. As a baseline, we apply SPM's MRI-based unified segmentation directly to the CT images. CTseg significantly outperformed this baseline for segmentation and normalisation, showed stronger TBV agreement, and achieved comparable TIV agreement. CTseg is freely available at https://github.com/WCHN/CTseg, and all experiment code is included in the repository for full reproducibility.

==> figures/table_prediction.tex <==
\begin{table}[t]
\centering
\small
\caption{Age and sex prediction from normalised tissue maps (10-fold CV, GP models, FWHM=8\,mm). Following the evaluation paradigm of \citet{brudfors2019superres}. Best value per column in bold; for Bias, smaller magnitude is better.}
\label{tab:prediction}
\small
\begin{tabular}{lcccccc}
\toprule
 & \multicolumn{4}{c}{Age regression} & \multicolumn{2}{c}{Sex classification} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-7}
Method & RMSE (yr) & SD (yr) & Bias (yr) & $r$ & Acc (\%) & AUC \\
\midrule
SPM-MR & 10.82 & 10.90 & -0.48 & 0.389 & 84.5 & 0.886 \\
SPM-CT & \textbf{10.30} & \textbf{10.39} & \textbf{0.04} & \textbf{0.449} & 86.2 & 0.869 \\
CTseg-CT & 10.52 & 10.62 & 0.06 & 0.436 & \textbf{87.9} & \textbf{0.920} \\
\bottomrule
\end{tabular}
\end{table}

